Accelerating Partial Evaluation in Distributed SPARQL Query Evaluation

Partial evaluation has recently been used for processing SPARQL queries over a large resource description framework (RDF) graph in a distributed environment. However, the previous approach is inefficient when dealing with complex queries. In this study, we further improve the "partial evaluation and assembly" framework for answering SPARQL queries over a distributed RDF graph, while providing performance guarantees. Our key idea is to explore the intrinsic structural characteristics of partial matches to filter out irrelevant partial results, while providing performance guarantees on a network trace (data shipment) or the computational cost (response time). We also propose an efficient assembly algorithm to utilize the characteristics of partial matches to merge them and form final results. To improve the efficiency of finding partial matches further, we propose an optimization that communicates variables' candidates among sites to avoid redundant computations. In addition, although our approach is partitioning-tolerant, different partitioning strategies result in different performances, and we evaluate different partitioning strategies for our approach. Experiments over both real and synthetic RDF datasets confirm the superiority of our approach.

==> overview.tex <==
\section{Overview}\label{sec:overview}

Figure \ref{fig:SystemArchitecture} illustrates the whole framework of our solution. In this paper, we are concerned with the challenge of efficiently answering SPARQL queries over LOD. We detail the different steps of the approach below.

\begin{figure}[h]
\begin{center}
    \includegraphics[scale=0.42]{pics/frame.pdf}
   \caption{\small Framework of Processing Distributed SPARQL Queries }
   \label{fig:SystemArchitecture}
\end{center}
\end{figure}


\textbf{Data Localization $\&$ Query Decomposition.} Given a SPARQL query $Q$, we localize relevant sources with regard to $Q$ and decompose $Q$ into some subqueries over different sources. For each triple pattern $t$ of $Q$, the control site sends ``SPARQL ASK'' queries to determine which sources contains results of $t$. Based on the returned results, we localize the relevant sources and decompose the query into some subqueries, where each subquery can be evaluated as a whole. Different from existing solutions, we propose a \underline{S}ource \underline{T}otology \underline{G}raph (STG) to further filter out relevant sources. 

\nop{
However, different from existing solutions, such as FedX \cite{DBLP:FedX}, we propose 

Like FedX \cite{DBLP:FedX}, the control site sends ``SPARQL ASK'' queries to determine which sources contains results of a query edge. According to the results of ``SPARQL ASK'' queries, we can localize the relevant sources and decompose the query into some subqueries, where each subquery can be evaluated as a whole.
}

Given a SPARQL query $Q$, after data localization and query decomposition, query $Q$ is decomposed to a set of subqueries $D=\{q_1@S_1,q_2@S_2,...,q_n@S_n\}$, where $S_i$ is a set of corresponding sources for subquery $q_i$, $i=1,...,n$.

\begin{example}\label{example:RDFAndSPARQL}
Figure \ref{fig:LocalizationAndDecomposition} shows the results of data localization and query decomposition for the example query in Figure \ref{fig:exampleRDF}(c).
\end{example}

\begin{figure}[h]
\begin{center}
    \includegraphics[scale=0.34]{pics/decomposition.pdf}
   \caption{\small Example of Data Localization $\&$ Query Decomposition}
   \label{fig:LocalizationAndDecomposition}
\end{center}
\end{figure}

\textbf{Dynamic Query Plan Generation $\&$ Query Execution.} In order to further improve the query performance, we propose a dynamic query plan generation approach. The query plan is dynamically constructed according to the intermediate results.  

\nop{
We propose a dynamic query plan 

 join order selection approach. Specifically, 

In this phase, the query optimization and execution are combined together. The query plan is dynamically constructed by the control site. The control site makes calls to the execution engine in sources for executing the subqueries. During optimization and execution, we introduce some pruning rules based on the source topology graph to filter out some irrelevant sources.
}

